Pore-network models and effective medium theory: A convergence analysis

The convergence between effective medium theory and pore-network modelling is examined. Electrical conductance on two and three-dimensional cubic resistor networks is used as an example of transport through composite materials or porous media. Effective conductance values are calculated for the networks using effective medium theory and pore-network models. The convergence between these values is analyzed as a function of network size. Effective medium theory results are calculated analytically and numerically. Pore-network results are calculated numerically using Monte Carlo sampling. The reduced standard deviations of the Monte Carlo sampled pore-network results are examined as a function of network size. Finally, a "quasi-two-dimensional" network is investigated to demonstrate the limitations of effective medium theory when applied to thin porous media. Power law fits are made to these data to develop simple models governing convergence. These can be used as a guide for future research that uses both effective medium theory and pore-network models.

==> Makefile <==
          NAME1 = diss
       PRODUCT1 = $(NAME1).pdf
     TEXSOURCE1 = $(NAME1).tex \
		    abstract.tex ack.tex glossary.tex intro.tex laysummary.tex \
		    ubcdiss.cls
           BBL1 = $(NAME1).bbl

#         NAME2 =
#      PRODUCT2 = $(NAME2).pdf
#    TEXSOURCE2 = $(NAME2).tex 
#          BBL2 = $(NAME2).bbl

      BIBINPUTS = biblio.bib

     PDFFIGURES = $(BUILTPDFFIGURES) ${PNGFIGURES}
     PNGFIGURES = 
     GIFFIGURES = 
     SVGFIGURES = 
# Following is for Berkeley Make syntax:
#BUILTPDFFIGURES = \
#		    ${PNGFIGURES:C/\.png/.pdf/g} \
#		    ${GIFFIGURES:C/\.gif/.pdf/g} \
#		    ${SVGFIGURES:C/\.svg/.pdf/g}

all: doc.pdf $(PRODUCT1)

$(NAME1).pdf: $(TEXSOURCE1) $(BBL1) $(PDFFIGURES)
$(NAME1).dvi: $(TEXSOURCE1) $(BBL1) $(EPSFIGURES)
$(NAME1).bbl: $(TEXSOURCE1) $(BIBINPUTS) $(PDFFIGURES)

#$(NAME2).pdf: $(TEXSOURCE2) $(BBL2) $(BUILTPDFFIGURES)
#$(NAME2).dvi: $(TEXSOURCE2) $(BBL2) $(BUILTEPSFIGURES)
#$(NAME2).bbl: $(TEXSOURCE2) $(BIBINPUTS) $(BUILTEPSFIGURES) $(BUILTPDFFIGURES)

clean:
	$(RM) ${BUILTPDFFIGURES} $(NAME1).aux $(NAME1).dvi \
	    $(NAME1).log $(NAME1).blg $(NAME1).bbl $(NAME1).out \
	    $(NAME1).toc $(NAME1).lof $(NAME1).lot $(NAME1).brf \
            *.aux

# configuration issues
.SUFFIXES: .tex .pdf .bbl

PDFLATEX=	pdflatex
BIBTEX=		bibtex
XELATEX=	xelatex 
LATEX=		latex
BIBLATEX=	$(PDFLATEX)
BIBTEX=		bibtex -min-crossref=1000
RM=		rm -f
MV=		mv
CP=		cp -p

.tex.pdf:
	$(PDFLATEX) $(LATEXFLAGS) $<
	@while egrep -q 'LaTeX Warning:.*Rerun|Rerun to get' $*.log; do \
	       echo $(PDFLATEX) $<; \
	      $(PDFLATEX) $(LATEXFLAGS) $< || exit $$?; \
	done

.tex.bbl: 
	$(BIBLATEX) $(LATEXFLAGS) $<
	$(BIBTEX) $*
	$(RM) $*.aux $*.dvi $*.pdf

doc.pdf: diss.pdf
	$(CP) diss.pdf doc.pdf

